Data.Readme: Documenting Table Relationships for Diverse Data Tasks

Large language models (LLMs) can perform diverse data tasks when given a small set of relevant tables. However, for complex tasks requiring multiple tables over large data lakes, identifying relevant tables for the task becomes a prerequisite, but remains challenging. This is because there are often many tables in a data lake with similar table and schema names, and limited additional semantic context, thereby forcing agents to spend substantial time exploring tables at online query time, greatly affecting models' ability to perform tasks accurately, while increasing cost/latency substantially. We present Data.Readme, a novel table documentation approach that uses lightweight offline processing to infer and index rich \emph{table-to-table relationships}, including confusable, joinable, and union-able tables. We further develop a suite of agentic tools for LLMs to work with the index, to help agents retrieve relevant tables and perform tasks much more efficiently and effectively. Finally, we study how to optimize our index construction with a budget constraint. On data lakes containing up to 12K tables, Data.Readme improves task accuracy by as much as 40 percentage points across a range of data discovery, data analysis, and data science tasks, outperforming diverse baselines, including powerful coding agents with unlimited time and monetary budgets. We also show that equipping existing methods (such as coding agents) with Data.Readme can not only lead to consistent quality gains, but also significantly reduce their latency by up to 6x, demonstrating the potential of Data.Readme.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> plan.tex <==
\section{Plan / Note}

Status reflects the verified scope in the current draft:
\done{} is complete, partial has remaining
coverage, and todo awaits matching results. \textit{can skip} denotes optional
low-priority work. A \textcolor{red}{$\times$}
marks a blocked baseline; the shared reason is stated in the table.
Repeated notes are consolidated.

\iftoggle{full}
{
    \yeye{Online setting (with QL) is \done{}: augmented BIRD/Spider bar charts are included in
    Section~\ref{sec:online-setting}; the without-QL control uses historical measurements.}
    \yeye{The same section includes completed fixed-table snippet and full-agent
    top-5 SQL/generated-NL contrasts, with their distinct protocols and controls.}
    \yeye{Inline snippet visibility and the completed SQL-only k sweep are also
    included: BIRD k=1/5/10/20, Spider k=1/5/10, with unchanged reused k=5 records.}
    \yeye{BCTD is evaluated at $k=10,50,100,150,200$,
    with $m=1000$ tier-distributed known requests in
    Section~\ref{sec:budget-experiments}. All 14 conditions share
    BIRD/Spider 609/274 questions and their respective 597/911-table
    raw pools. Known All-cover and Dataset full are distinct references.
    Spider meets the full-minus-three-point target at $k=150$;
    BIRD does not at $k\le200$. Unknown fees remain unknown.
    Isolated selection-runtime scaling and repeated-run studies remain follow-ups;
    fixed-README repeats are not included.}
    
    \readmeresulttable{plan_notes}
      {Plan / Note: verified scope and remaining work.}
      {tab:plan-notes}
    \FloatBarrier
}
{
}
